Uncertainty-aware Evaluation of Auxiliary Anomalies with the Expected Anomaly Posterior

Anomaly detection is the task of identifying examples that do not behave as expected. Because anomalies are rare and unexpected events, collecting real anomalous examples is often challenging in several applications. In addition, learning an anomaly detector with limited (or no) anomalies often yields poor prediction performance. One option is to employ auxiliary synthetic anomalies to improve the model training. However, synthetic anomalies may be of poor quality: anomalies that are unrealistic or indistinguishable from normal samples may deteriorate the detector's performance. Unfortunately, no existing methods quantify the quality of auxiliary anomalies. We fill in this gap and propose the expected anomaly posterior (EAP), an uncertainty-based score function that measures the quality of auxiliary anomalies by quantifying the total uncertainty of an anomaly detector. Experimentally on 40 benchmark datasets of images and tabular data, we show that EAP outperforms 12 adapted data quality estimators in the majority of cases.

==> neurips2024/texfiles/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
%The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page limit. 

%Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
%\begin{itemize}
%    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
%\end{itemize}

%{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

%The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

%IMPORTANT, please:
%\begin{itemize}
%    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
%\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We make two claims. First, we claim that our approach outperforms 12 baselines in the majority of cases, which we show in \Cref{sec:exp}. Second, we claim that our method ranks the anomalies as (1st) realistic, (2nd) unrealistic, and (3rd) indistinguishable, which we show in \Cref{sec:theory}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We detailed the key assumptions of the methodology in \Cref{sec:method} and \Cref{sec:theory}, as well as the general limitations in \Cref{sec:conclusion_and_limitations}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by , \answerNo{}, or \answerNA{}.
    \item[] Justification: \Cref{sec:theory} illustrates our main result and provides a complete proof. The properties can be quickly derived from basic calculus and limits.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \Cref{sec:exp} gives all details on our experimental setup, including the preprocessing of the data, the model's hyperparameters, and the procedure to correctly set the experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We will release the code upon acceptance. The data is publicly available. The experimental section provides all the details to reproduce the results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \Cref{sec:exp} provides all details.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \Cref{tab:mean_pm_std} in the Supplement shows the aggregated results in terms of mean $\pm$ standard deviation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \Cref{sec:exp} (setup) gives all details.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We are aware of the code of ethics and do not violate any clause.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \Cref{sec:conclusion_and_limitations} provides our statement on the societal impact.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not have risks for misuse to the best of our knowledge.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Only the authors contributed to this paper. The license has been selected for submission in OpenReview.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Code will be released upon acceptance, along with the framework to use it.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


==> neurips2024/texfiles/conclusion.tex <==
\section{Conclusion and Limitations}\label{sec:conclusion_and_limitations}
This paper addressed the problem of evaluating the quality of an auxiliary set of synthetic anomalies. With this quality score, one can enrich an anomaly detection dataset to learn a more accurate anomaly detector. 
We proposed the expected anomaly posterior (\ourmethod{}), the first quality score function for auxiliary anomalies derived from an approximation for the posterior over the probability that a given input is an anomaly.
We showed that our approach theoretically assigns higher scores to the realistic anomalies, compared to unrealistic and indistinguishable anomalies. Empirically, we investigated how \ourmethod{} compares to adapted data quality estimators at (1) assigning quality scores, (2) using such scores to enrich the data for training, and (3) model selection. On $40$ datasets, we show that \ourmethod{} outperforms all $12$ baselines in the majority of the cases.

\paragraph{Limitations.} While our theoretical categorization refers to general anomalies, the concept of unrealistic/indistinguishable might be domain-driven and require adjustments in some applications (e.g., scratches on fabrics are unrealistic but would get high quality). Also, uncertainty-based methods require limited training samples to be effective and one may need to reduce the training normals.

\paragraph{Impact Statement.} This paper presents work whose goal is to advance the field of Machine Learning. There are many potential societal consequences of our work, none of which we feel must be specifically highlighted here.


==> neurips2024/texfiles/experiments.tex <==
\section{Experiments}\label{sec:exp}

We empirically evaluate three aspects of our method \ourmethod{}: (a) whether it measures properly the quality of auxiliary anomalies, and (b) its impact on selecting auxiliary anomalies for learning a model or (c) for model selection. To this end, we address the following five experimental questions:

\begin{itemize}[nolistsep]
    \item[Q1.] How does \ourmethod{} compare to existing methods at assigning quality scores?
    \item[Q2.] How does a model’s performance vary when including \emph{high-quality} anomalies for training?
    \item[Q3.] How does a model’s performance vary when including \emph{low-quality} anomalies for training?
    \item[Q4.] How does the performance of a CLIP-based zero-shot anomaly detection method vary when using the selected auxiliary anomalies for prompt tuning?
    \item[Q5.] How do \ourmethod{}' scores vary for different priors?
\end{itemize}

\subsection{Experimental Setup}


\paragraph{Baselines.}
We compare \ourmethod{}\footnote{Code is available at: URL provided upon acceptance.} with $12$ adapted baselines:
\textsc{Loo}, \textsc{kNNShap}~\cite{jia2019efficient}, \textsc{DataBanzhaf}~\cite{wang2023data}, \textsc{AME}~\cite{lin2022measuring}, \textsc{LavaEv}~\cite{just2023lava}, \textsc{Inf}~\cite{feldman2020neural}, and \textsc{DataOob}~\cite{kwon2023data} are existing data quality evaluators that measure the impact of a training example on the model performance. We adapt these methods by including each auxiliary anomaly (individually) in the training set and evaluating its contribution. \textsc{RandomEv} assigns uniform random scores to each auxiliary anomaly. \textsc{Rarity}~\cite{han2022rarity} computes the rarity score of each auxiliary anomaly. Finally, we include the estimators for the data density $P_x$, the class conditional probability $P_{y|x}$, and a linear combination of them $P_{y|x}+ NP_x$.

\paragraph{Data.}

We carry out our study on $40$ datasets, including $15$ widely used benchmark image datasets (\textsc{MvTec})~\cite{bergmann2019mvtec}, $3$ industrial image datasets for Surface Defect Inspection (SDI)~\cite{Wang_2022_BMVC}, and an additional $22$ benchmark tabular datasets for anomaly detection with semantically useful anomalies, commonly referenced in the literature~\cite{han2022adbench}. These datasets vary in size, feature count, and anomaly proportion.

For each dataset, we construct an auxiliary set of $l$ anomalies by combining realistic, indistinguishable, and unrealistic anomalies ($\frac{l}{3}$ each). Realistic anomalies are labeled anomalies provided with the dataset, indistinguishable anomalies are labeled normal examples with swapped labels, and unrealistic anomalies come from other datasets. Specifically, to collect unrealistic anomalies we randomly select $5$ datasets out of the $40$, subsample them to a specific example count, and fix their dimensionality to $d$ using random projections (either extending or reducing it). \emph{Pseudo-quality} labels ``good'' and ``poor'' are assigned to real anomalies and the other two groups, respectively, reflecting the ground truth where real anomalies should have high-quality scores.


%We carry out our study on $40$ datasets: $15$ commonly used benchmark \emph{image} datasets (MvTec)~\cite{bergmann2019mvtec}, $3$ datasets of industrial images for Surface Defect Inspection (SDI)~\cite{Wang_2022_BMVC}, and additionally $22$ benchmark \emph{tabular} datasets for anomaly detection, which contain semantically useful anomalies and are widely used in the literature~\cite{campos2016evaluation,han2022adbench}. All datasets vary in size, number of features, and proportion of anomalies. The Supplement~\ref{sec:supplement} provides further details.

%For each dataset, we create one auxiliary set of $l$ anomalies by combining real, indistinguishable, and unrealistic anomalies ($\frac{l}{3}$ each). The real anomalies are the labeled examples provided with the dataset. The indistinguishable anomalies are labeled normal examples with the swapped label. The unrealistic anomalies are external examples coming from different datasets: (i) we randomly pick $5$ other datasets (out of the $40$), (ii) we randomly subsample them to collect a specific amount of examples, and (iii) we fix their dimensionality to $d$ (either extending it or reducing it) using random projections. We provide the pseudo-label ``good'' to the real anomalies, and ``poor'' to the other two groups. This reflects the ground truth, where real anomalies should have high-quality scores.


\paragraph{Setup.}
For each dataset, we proceed as follows: 
% (i) We randomly split the anomalies into training ($10\%$), auxiliary ($40\%$), and test ($50\%$) sets, with $\frac{l}{3} = 40\%$ of available anomalies;
(i) We create a balanced test set by adding random normal examples and $50\%$ of available anomalies; 
(ii) We generate a set of $l$ auxiliary anomalies as described above with $\frac{l}{3} = 40\%$ of available anomalies;
(iii) We create a training set by adding $10\%$ of available anomalies and all remaining normal examples to the training set.
(iv) We apply all methods to evaluate the external set of anomalies, using the training set for validation when required (as $m \ll n$, we avoid partitioning the training set); 
%(v) We compute the six metrics to compare \ourmethod{} with the baselines. 
To mitigate noise, steps (i)-(iv) are repeated $10$ times with different seeds, resulting in a total of $4000$ experiments (datasets, methods, seeds). While computing \ourmethod{} is fast, the baselines have high computational costs because they train a model several times. To run all experiments, we use an internal cluster of six 24- or 32-thread machines (128 GB of memory). The experiments finish in $\sim 72$ hours.

%For each of the $40$ datasets, we proceed as follows: 
%(i) randomly split the available anomalies into training/auxiliary/test set following the proportions $10/40/50$ (thus, $\frac{l}{3}$ is $40\%$ of the available anomalies);
%(ii) include a random sample of normals to the test set such that the classes are balanced, create the synthetic auxiliary set of $l$ anomalies as explained before, and include all remaining normals to the training set; 
%(iii) apply all methods to evaluate the external set of anomalies leveraging the training set as validation whenever a baseline needs it;\footnote{Because $m \ll n$, we do not partition the training set.}
%(iv) evaluate each method's quality scores by measuring the \textbf{AUROC$_{\textsc{qs}}$} and \textbf{\textsc{Acc}};
%(v) use the methods' ranking of the auxiliary anomalies to compute the LC, and measure \textbf{AULC$_{\frac{1}{3}}$}, \textbf{LC$_{\frac{1}{3}}$} (following the metrics' ordering), and \textbf{AULC$_{\frac{2}{3}}$}, \textbf{LC$_{\frac{2}{3}}$} (following their inverse ordering). To average out the noise, we repeat all steps (i)-(v) $10$ times with different seeds. We carry out a total of $40\times10\times10 = 4000$ experiments (dataset, method, seed).


\paragraph{Models and Hyperparameters.}
For all baselines, we use \textsc{SSDO}~\cite{vercruyssen2018semi} as the underlying anomaly detector $f$ with $k=10$ and Isolation Forest~\cite{liu2008isolation} as prior. When exposed to selected auxiliary anomalies, we employ an \textsc{SVM} with RBF kernel (for images) and a \textsc{Random Forest} (for tabular data) to make the normal vs. abnormal classification. For images, we use the pre-trained \textsc{ViT-B-16-SigLIP}~\cite{zhai2023sigmoid} to extract the features from images and use them as inputs to \ourmethod{} and all baselines.
Our method \ourmethod{} has one hyperparameter, namely the prior $\alpha_0, \beta_0$, which we set to $\frac{m}{n}$ (the proportion of anomalies in the training set) and $1-\frac{m}{n}$. Intuitively, this corresponds to the expected proportion of (real) anomalies if an external dataset was sampled from $\Pp(X,Y)$. The baselines\footnote{Code: \url{https://github.com/opendataval}} have the following hyperparameters: \textsc{kNNShap} and \textsc{Rarity} have $k=10$, \textsc{DataBanzhaf}, \textsc{AME}, \textsc{Inf} and \textsc{DataOob} use $50$ models. All other hyperparameters are set as default~\cite{soenen2021effect}.

\paragraph{Evaluation Metrics.}
We employ \textbf{four} evaluation metrics. First, we use the Area Under the Receiving Operator Curve (\textbf{AUC$_{\textsc{qlt}}$}) to evaluate the methods' ability to rank good-quality examples higher than poor-quality ones based on quality scores compared to the pseudo-quality labels. %Secondly, we measure accuracy (\textbf{ACC$_{\textsc{qlt}}$}) by classifying the top $\frac{1}{3}$ of scores as ``good'' and the rest as ``poor'' and compare these predictions with pseudo-quality labels. 
Second, we qualitatively analyze the impact of using auxiliary anomalies in training a model, showing the learning curves (\textbf{LC$_{\textsc{g}}$}) with the number of added anomalies following the ranking of quality scores on the x-axis and the test accuracy on the y-axis. We compute the area under the learning curve up to $\frac{1}{3}$ of ranked anomalies (\textbf{AULC$_{\textsc{g}}$}) and the test accuracy after including top $\frac{1}{3}$ of ranked anomalies (\textbf{ACC$_{\textsc{g}}$}). Similarly, we compute the \textbf{LC$_{\textsc{p}}$} following the methods' inverse ordering and measure the \textbf{AULC$_{\textsc{p}}$} of including up to $\frac{2}{3}$ of inversely-ranked anomalies, where lower values are desirable. Also, rankings from $1$ (best) to $13$ (worst) are assigned for each method in every experiment, which are denoted by a $r$ in front in Table~\ref{tab:aggregated_results}.

%We use \textbf{six} evaluation metrics to measure the performance of the methods. First, we measure the Area Under the Receiving Operator Curve (\textbf{AUROC$_{\textsc{qs}}$}) between the quality scores and the pseudo-label (good/poor), which captures the ability of the methods to rank good-quality examples higher than the poor-quality ones. Second, we threshold the quality scores such that each method predicts ``good'' for the top $\frac{1}{3}$ of its scores, and ``poor'' for the remaining and measure the accuracy (\textbf{\textsc{Acc}}) between these predictions and the true pseudo-labels. Third, we measure the impact of using the synthetic anomalies to train a binary classification model. For this task, we sort each method's quality scores in descending order and include, one at a time, the synthetic anomalies following such ranking. This enables us to plot the \emph{learning curve} (LC): on the x-axis, the number of auxiliary anomalies added to the training set, and, on the y-axis, the accuracy of the model trained with the correspondent extended training set. We use the plots for qualitative analysis, and measure (1) the area under the learning curve up to including $\frac{1}{3}$ of auxiliary anomalies (\textbf{AULC$_{\frac{1}{3}}$}) and (2) the test accuracy after including the $\frac{1}{3}$ of examples (\textbf{LC$_{\frac{1}{3}}$}). Because high quality anomalies have a larger impact on the test performance, the higher the area the better. With a similar idea, we compute the LC following the inverse ordering (i.e., ascending scores) and compute its area when including up to $\frac{2}{3}$ of synthetic anomalies (\textbf{AULC$_{\frac{2}{3}}$}) and the LC value (\textbf{LC$_{\frac{2}{3}}$}). This time, the lower the values the better, as only low-quality examples are included. For each of the previous metrics, we rank all methods in each experiment from $1$ (best method) to $10$ (worst method). We indicate such values by $^r$. Table~\ref{tab:aggregated_results} illustrates the aggregated results.
\input{tables/main_results}
\subsection{Experimental Results}

% \begin{table*}[htpb]
% \label{tab:aggregated_results}
% \setlength{\tabcolsep}{2.0pt}
% \centering
% \small
% \caption{Summary of the results obtained by the $10$ methods over $18$ image (above) and $22$ tabular (below) datasets. The columns $2-7$ represent the $6$ performance metrics employed, while the columns $8-13$ show their ranking values and the last column averages all the rankings together. For metrics desiring lower values, we mark with a $\downarrow$. Overall, \ourmethod{} achieves the best performance and ranking position for most evaluation metrics (for both image and tabular data) as well as the best average ranking (last column).}
%      \resizebox{\linewidth}{!}{ 
% \begin{tabular}{l|c|c|c|c|c|c||c|c|c|c|c|c||c}
% \multicolumn{14}{c}{\bf{\textsc{18 Image Datasets}}}\\
% \toprule
% \textsc{Evaluator} & \textbf{AUC$_{\textsc{qlt}}$} & \textbf{ACC$_{\textsc{qlt}}$} & \textbf{AULC$_{\textsc{g}}$} & \textbf{ACC$_{\textsc{g}}$} & \textbf{AULC$_{\textsc{p}}$}($\downarrow$) & \textbf{ACC$_{\textsc{p}}$}($\downarrow$) 
% & \textbf{AUC$_{\textsc{qlt}}^r$} & \textbf{ACC$_{\textsc{qlt}}^r$} & \textbf{AULC$_{\textsc{g}}^r$} & \textbf{ACC$_{\textsc{g}}^r$} & \textbf{AULC$_{\textsc{p}}^r$} & \textbf{ACC$_{\textsc{p}}^r$} & \textbf{\textsc{Avg$^r$}} \\
% \midrule
% \bf{\ourmethod{}} & \bf{0.803} & \bf{0.770} & \bf{0.717} & \bf{0.833} & 0.688 & \bf{0.748} & \bf{1.88} & \bf{1.87} & \bf{3.40} & \bf{2.75} & \bf{2.86} & \bf{1.63} & \bf{2.40} \\
% \textsc{Rarity} & 0.681 & 0.711 & 0.698 & 0.786 & 0.738 & 0.788 & 3.43 & 2.62 & 4.22 & 4.54 & 5.96 & 3.06 & 3.97 \\
% \textsc{Lava} & 0.742 & 0.665 & 0.665 & 0.755 & 0.709 & 0.794 & 2.28 & 3.31 & 6.81 & 6.35 & 3.67 & 3.49 & 4.31 \\
% \textsc{Loo} & 0.537 & 0.434 & 0.693 & 0.777 & 0.694 & 0.840 & 5.75 & 7.62 & 5.04 & 5.76 & 4.56 & 6.82 & 5.93 \\
% \textsc{RandomEv} & 0.491 & 0.557 & 0.696 & 0.793 & 0.756 & 0.830 & 7.10 & 4.97 & 5.29 & 5.26 & 7.45 & 6.42 & 6.07 \\
% \textsc{DataBanzhaf} & 0.500 & 0.551 & 0.668 & 0.775 & 0.748 & 0.833 & 6.90 & 5.00 & 6.81 & 5.77 & 6.44 & 5.93 & 6.14 \\
% \textsc{Inf} & 0.488 & 0.540 & 0.681 & 0.778 & 0.744 & 0.838 & 7.02 & 5.24 & 6.01 & 5.88 & 6.49 & 6.47 & 6.19 \\
% \textsc{kNNShap} & 0.509 & 0.434 & 0.695 & 0.794 & 0.754 & 0.831 & 6.88 & 7.91 & 5.40 & 5.21 & 7.08 & 6.17 & 6.44 \\
% \textsc{AME} & 0.512 & 0.383 & 0.693 & 0.793 & 0.756 & 0.833 & 6.84 & 8.65 & 5.47 & 5.13 & 7.48 & 6.36 & 6.68 \\
% \textsc{DataOob} & 0.505 & 0.398 & 0.685 & 0.739 & \bf{0.668} & 0.874 & 6.91 & 7.82 & 6.59 & 8.32 & 3.07 & 8.61 & 6.88 \\
% \midrule
% \multicolumn{14}{c}{\bf{\textsc{22 Tabular Datasets}}}\\
% \midrule
% \bf{\ourmethod{}} & \bf{0.821} & \bf{0.776} & 0.779 & \bf{0.839} & \bf{0.717} & \bf{0.800} & \bf{1.66} & \bf{1.74} & 3.85 & \bf{3.72} & \bf{1.59} & \bf{2.45} & \bf{2.50} \\
% \textsc{Rarity} & 0.724 & 0.709 & \bf{0.782} & \bf{0.839} & 0.753 & 0.810 & 2.87 & 2.38 & \bf{3.82} & 4.19 & 3.52 & 3.14 & 3.32 \\
% \textsc{Lava} & 0.723 & 0.667 & 0.744 & 0.794 & 0.747 & 0.839 & 2.96 & 3.23 & 6.41 & 5.98 & 2.97 & 4.00 & 4.26 \\
% \textsc{RandomEv} & 0.502 & 0.557 & 0.773 & 0.827 & 0.809 & 0.859 & 6.27 & 4.37 & 4.34 & 4.64 & 7.03 & 6.31 & 5.49 \\
% \textsc{kNNShap} & 0.541 & 0.395 & 0.770 & 0.825 & 0.805 & 0.859 & 5.84 & 8.31 & 4.58 & 4.55 & 6.59 & 6.10 & 5.99 \\
% \textsc{Loo} & 0.504 & 0.388 & 0.750 & 0.798 & 0.792 & 0.858 & 5.97 & 7.85 & 5.80 & 5.97 & 5.49 & 6.18 & 6.21 \\
% \textsc{AME} & 0.498 & 0.339 & 0.772 & 0.827 & 0.809 & 0.861 & 6.53 & 9.21 & 4.45 & 4.68 & 7.10 & 6.49 & 6.39 \\
% \textsc{DataOob} & 0.513 & 0.468 & 0.729 & 0.768 & 0.785 & 0.862 & 6.52 & 6.51 & 7.93 & 8.23 & 5.21 & 6.38 & 6.79 \\
% \textsc{Inf} & 0.434 & 0.506 & 0.742 & 0.795 & 0.816 & 0.865 & 7.91 & 5.44 & 6.59 & 6.20 & 7.69 & 6.99 & 6.81 \\
% \textsc{DataBanzhaf} & 0.415 & 0.492 & 0.736 & 0.789 & 0.817 & 0.866 & 8.45 & 5.95 & 7.24 & 6.88 & 7.80 & 7.00 & 7.22 \\
% \bottomrule
% \end{tabular}}
% \end{table*}

\paragraph{Q1. \ourmethod{} vs baselines at assigning quality scores.} 


Figure~\ref{fig:q1_auroc_qs} shows the methods' mean AUC$_{\textsc{qlt}}$ on both image (left) and tabular data (right). On images, \ourmethod{} outperforms all baselines on $13$ out of $18$ datasets, achieving an average AUC$_{\textsc{qlt}}$ significantly higher than \textsc{Lava} and \textsc{Rarity} by $6$ and $12$ percentage points, as shown in Table~\ref{tab:aggregated_results}. Also, \ourmethod{} consistently obtains the lowest (best) average ranking positions ($1.99$ for rAUC$_{\textsc{qlt}}$). On tabular data, \ourmethod{} 
obtains an average AUC$_{\textsc{qlt}} = 0.821$, which is around $10$ percentage points higher than the runner-ups. Also, \ourmethod{} outperforms \textsc{Lava} and \textsc{Rarity} on $18$ and $17$ datasets and obtains the best average ranking ($1.91$).

%performs better or equal to \textsc{Lava} and \textsc{Rarity} on, respectively, $18$ and $17$ datasets, obtains the best average ranking ($1.91$) and surpasses both the runner-ups by almost $10$ percentage points on AUC$_{\textsc{qlt}}$ ($0.821$). 

Interestingly, only \ourmethod{}, \textsc{Lava}, \textsc{Rarity}, and $P_{y|x}+NP_x$ achieve performance better than random, while other methods get average AUC$_{\textsc{qlt}}$ around $0.5$, which highlights their inability to distinguish good and poor auxiliary anomalies consistently. As a second remark, \ourmethod{} performs lower than random for the dataset \textsc{Tile}. This happens because the defective images are extremely different than the normal images, thus resulting in real anomalies falling in zero-density regions, which our method would categorize as unrealistic.

%Figure~\ref{fig:q1_auroc_qs} shows the mean AUC$_{\textsc{qs}}$ for all methods on both image (left) and tabular data (right). On images, \ourmethod{} outperforms all baselines on $13$ out of $18$ datasets, obtaining an average AUC$_{\textsc{qs}}$ that is higher than the runner-ups \textsc{Lava} and \textsc{Rarity} by more than, respectively, $6$ and $12$ percentage points. Similarly, \ourmethod{} achieves an average accuracy \textsc{Acc} that is higher, on average, by around $10$ and $6$ percentage points, compared to the runner-ups. 
%Table~\ref{tab:aggregated_results} shows the aggregated results. Moreover, the columns AUC$_{\textsc{qs}}^r$ and \textsc{Acc}$^r$ show that \ourmethod{} obtains the lowest (best) average ranking positions ($1.88$ and $1.87$), which are substantially lower than \textsc{Lava}'s ($2.28$, $3.31$) and \textsc{Rarity}'s ($3.43$, $2.62$) ones. Specifically, \ourmethod{} ranks as the first (best) baseline on $130$ (for AUC$_{\textsc{qs}}$) and $121$ (for \textsc{Acc}) experiments out of $180$, while the runner-ups obtain the first position only in, respectively, $23-6$ and $20-34$ experiments (for AUC$_{\textsc{qs}}$-\textsc{Acc}).

%For tabular datasets, Figure~\ref{fig:q1_auroc_qs} (right) shows that \ourmethod{} performs better or equal (i.e., difference $\le 0.01$) than \textsc{Lava} and \textsc{Rarity}, respectively, on $18$ and $17$ datasets out of $22$, with an average AUC$_{\textsc{qs}}$ of $0.821$ that is higher than the two runner-ups' performances by around $10$ percentage points. Similarly to image data, \ourmethod{} shows a large gap (between $7$ and $11$ percentage points) on the accuracy when compared to \textsc{Rarity} and \textsc{Lava}. Moreover, it obtains the lowest ranking position for both AUC$_{\textsc{qs}}$-\textsc{Acc} metrics ($1.66$, $1.74$), classifying in the top-$2$ of the ranking on more than $180$ experiments out of $220$.

%Finally, we want to make two relevant remarks. First, only \ourmethod{}, \textsc{Lava} and \textsc{Rarity} achieve a performance better than random. All other methods have an average AUC$_{\textsc{qs}}$ and \textsc{Acc} around $0.5$, which makes them unable to split good and poor auxiliary anomalies consistently. Second, \ourmethod{} gets a performance lower than random for the dataset \textsc{tile}. This happens because the defective images are much different than the normals, thus resulting in real anomalies that fall in zero-density regions, which our method would categorize as unrealistic.

\begin{figure*}[t!]
%\vspace{.1in}
\centerline{\includegraphics[width=\textwidth]{imgs/240401_comparison_aucsplit.pdf}}
\vspace{-.12in}
\caption{The plot illustrates the average AUC$_{\textsc{qlt}}$ obtained by each method on a per-dataset basis (left for image data, right for tabular data). \ourmethod{} achieves the highest (best) performance for most datasets, beating the runner-ups \textsc{Rarity} and \textsc{Lava} on, respectively, $30$ and $31$ datasets out of $40$.
}\label{fig:q1_auroc_qs}
\vspace{-.03in}
\end{figure*}

\begin{figure*}[t!]
%\vspace{.1in}
\centerline{\includegraphics[width=\textwidth]{imgs/240401_aucl_curves.pdf}}
\vspace{-.12in}
\caption{Learning curve (LC) obtained by following the method's ordering (top) and inverse ordering (bottom) for five representative image datasets. Top: \ourmethod{}' LC$_{\textsc{g}}$ grows sooner (i.e., better) than the other methods', which confirms that including high-quality anomalies in the training set has a larger impact on the test performance. Bottom: \ourmethod{}' LC$_{\textsc{p}}$ rises later (i.e., better) than most baselines', showing that low-quality anomalies have a comparatively modest impact on the test performance.
}\label{fig:q2_aucl}
\vspace{-.03in}
\end{figure*}

\paragraph{Q2. Including high-quality anomalies in training.}

We measure how the performance of a model varies when introducing the top $\frac{1}{3}$ of auxiliary anomalies into the training following the methods' rankings. Figure~\ref{fig:q2_aucl} (top) shows the learning curves (LC$_{\textsc{g}}$) for five representative image datasets. Overall, including high-ranked anomalies first has the claimed impact on the model's performance: the learning curve grows sooner for \ourmethod{} compared to all baselines. Consequently,  \ourmethod{} obtains an AULC$_{\textsc{g}}$ that is, on average, higher than all the baselines by between $2$ (vs. \textsc{Rarity} and $P_{y|x}+NP_x$) and $5$ (vs. \textsc{Lava}) percentage points. After including one-third of the auxiliary anomalies for training, \ourmethod{} shows an average improvement on the test performance (ACC$_{\textsc{g}}$) of $4$ to $10$ points over all baselines, standing out as the only method significantly better than \textsc{RandomEv}.
Moreover, Table~\ref{tab:aggregated_results} shows that \ourmethod{} achieves the best average ranking for both AULC$_{\textsc{g}}$ (i.e., $3.94$) and ACC$_{\textsc{g}}$ (i.e., $3.12$).

On tabular data, Table~\ref{tab:aggregated_results} shows that \ourmethod{} achieves an average AULC$_{\textsc{g}}$ slightly lower than \textsc{Rarity} ($0.779$ vs $0.782$) and a similar ACC$_{\textsc{g}}$ (both $0.839$). This occurs because, for most tabular datasets, \textsc{Rarity} assigns high-quality scores to the unrealistic anomalies which are obviously different than normal data. When including them for training, it yields an improvement of the \textsc{Random Forest}'s test accuracy surprisingly. From a ranking perspective, \ourmethod{} obtains the lowest (best) average with rAULC$_{\textsc{g}} = 4.27$ (vs. \textsc{Rarity}'s $4.42$), and rACC$_{\textsc{g}} = 4.28$ (vs. \textsc{Rarity}'s $4.91$).

\input{tables/prompt_tuning}

\paragraph{Q3. Including low-quality anomalies in training.}
Figure~\ref{fig:q2_aucl} (bottom) shows the LC$_{\textsc{p}}$ obtained by following an inverse ordering of the methods, i.e., lower ranked anomalies are included first. Using this inverse ordering should result in much slower growth of the LC$_{\textsc{p}}$s: in some cases, the test accuracy using \ourmethod{} remains stable (\textsc{Capsule}, \textsc{Metalnut}, \textsc{Screw}), while in others it shows strong fluctuations going up and down quickly (\textsc{Pill}). Interestingly, every baseline's performance goes up for \textsc{Tile}: this is due to their poor ability to assign scores for this dataset, as described in Q1. Surprisingly, \textsc{DataOob} obtains the lowest (best) AULC$_{\textsc{p}}$, while \ourmethod{} has the second best AULC$_{\textsc{p}}$ with just two percentage points as gap. However, when ranking the experiments, \ourmethod{} achieves the best average ranking ($3.66$ of rAULC$_{\textsc{p}}$), thus being the preferred method for most of the experiments. %More importantly, \ourmethod{} outperforms all baselines when measuring LC$_{\frac{2}{3}}$, the value of the LC after including $\frac{2}{3}$ of the auxiliary anomalies: with a performance of $0.748$, it improves upon \textsc{DataOob} by more than $12$ percentage points. Additionally, it shows the best average ranking LC$_{\frac{2}{3}}^r$, by substantially improving over the runner-up \textsc{Rarity} ($1.63$ vs $3.06$).

On tabular data, the results confirm the previous analysis: \ourmethod{} has the lowest AULC$_{\textsc{p}}$ on $137$ experiments out of $220$, while \textsc{Rarity} and \textsc{Lava} achieve so only on, respectively, $29$ and $31$ experiments. This motivates that \ourmethod{} obtains an average AULC$_{\textsc{p}}$ that is better than all baselines by between $3$ and $10$ percentage points, as shown in Table~\ref{tab:aggregated_results}.

\paragraph{Q4. Prompt tuning for zero-shot anomaly detection.}
CLIP-based anomaly detection methods save the effort of collecting training examples and enable a zero-shot anomaly detection~\cite{jeong2023winclip}. However, their detection performance depends on the choice of prompts, which is usually tuned by using labeled real-world anomalies.
We study the impact of selected auxiliary anomalies on prompt tuning for the \textsc{MvTec} datasets.
%\footnote{MVTEC dataset is an industrial anomaly detection dataset including 15 various classes.}. 
Specifically, we search a prompt for each object class achieving the best performance on the selected auxiliary anomalies from a pool of $27$ candidate prompts (see details in \Cref{app:prompts}), and apply the best-performing prompt to CLIP at test time.

\Cref{tab:prompt_tuning} reports the test AUCs of CLIP with the best-performing prompts selected by each data valuation method. We can see that \ourmethod{} performs the best on $12$ of $15$ classes and achieves the highest AUC averaged over all classes. Thanks to accounting for both the class conditional probability and the data density, \ourmethod{} clearly outperforms \textsc{Rarity} and $P_x$, which only consider the data density, $P_{y|x}$, which only considers the class conditional probability, and their naive linear combination $P_{y|x}+NP_x$.
The results confirm that \ourmethod{} selects high-quality auxiliary anomalies for the model selection purpose. We list the prompts selected by \ourmethod{} in \Cref{app:prompts}.

\paragraph{Q5. \ourmethod{}' sensitivity to $\frac{\alpha_0}{\alpha_0+\beta_0}$.} 

% \begin{table}[t!]
% \label{tab:hyperparams}
% \centering
% \small
% \caption{Comparison between \ourmethod{} with default $\alpha_0$ and its six variants \ourmethod{}$_w$ that set $\alpha_0=w, \beta_0=1-w$. Rankings show low sensitivity to such a choice, as long as $\alpha_0<0.4$.}
% \begin{tabular}{lcccc}
% \toprule
% \textsc{Evaluator} & \textbf{AUC$_{\textsc{qs}}^r$} & \textbf{LC$_{\frac{1}{3}}^r$} & \textbf{LC$_{\frac{2}{3}}^r$} & \textbf{\textsc{Avg$^r$}} \\
% \midrule
% \ourmethod{} & 2.92 & \bf{2.73} & \bf{2.51} & \bf{2.86} \\
% \ourmethod{}$_{0.2}$ & \bf{2.78} & 3.25 & 3.49 & 3.07 \\
% \ourmethod{}$_{0.3}$ & 3.39 & 3.40 & 4.10 & 3.19 \\
% \ourmethod{}$_{0.1}$ & 3.01 & 3.46 & 3.27 & 3.44 \\
% \ourmethod{}$_{0.05}$ & 3.63 & 3.78 & 3.30 & 3.77 \\
% \ourmethod{}$_{0.01}$ & 4.10 & 3.54 & 3.15 & 3.79 \\
% \ourmethod{}$_{0.4}$ & 4.71 & 4.79 & 5.83 & 4.54 \\
% \bottomrule
% \end{tabular}
% \end{table}


\ourmethod{} requires two hyperparameters: $\alpha_0$, $\beta_0$ of the prior Beta distribution. To remove one degree of freedom, we set $\alpha_0+\beta_0 = 1$ such that the dataset size $n$ is much stronger ($n$ times) than our initial belief. Then, we investigate how varying the parameter $\alpha_0 \in [0,0.5)$ impacts \ourmethod{}'s overall performance ($\beta_0 = 1-\alpha_0$). We compare seven versions of our method by setting $\alpha_0 \in \{0.01,0.05,0.1,0.2,0.3,0.4\}$, in addition to the original \ourmethod{} that leverages the contamination level $\alpha_0 = m/n$. We call \ourmethod{}$_{w}$ the variant that uses $\alpha_0 = w$. \Cref{tab:hyperparams} in the Supplement shows the rankings of these $7$ variants for AUC$_{\textsc{qlt}}$ and ACC$_{\textsc{g}}$ and their average. Overall, both parameters have a low impact on our method: while a higher value for $\alpha_0$ improves the AUC$_{\textsc{qlt}}$, in some experiments this improvement does not yield better performance at test time in terms of ACC$_{\textsc{g}}$. Moreover, setting $\alpha_0$ too high or too low has inherent risks: \ourmethod{}$_{0.4}$ and \ourmethod{}$_{0.01}$ are the worst variants by far, with significant drops in performance compared to the other variants.

==> neurips2024/texfiles/introduction.tex <==
\section{Introduction}

Anomaly detection aims at identifying the examples that do not conform to the normal behaviour~\cite{chandola2009anomaly}. Anomalies are often connected to adverse events, such as defects in production lines~\cite{wang2024improving}, excess water usage~\cite{perini2023estimating}, failures in petroleum extraction~\cite{marti2015anomaly}, or breakdowns in wind turbines~\cite{perini2022transferring}. Detecting anomalies in time can reduce monetary costs and protect resources from harm.
For this reason, there has been significant effort to develop data-driven methods for anomaly detection.

%\changed{Unfortunately, having access to a representative set of anomalous examples is usually challenging for two reasons. First, one may need to acquire huge loads of data before collecting an anomaly, as they are rare and sparse events. For instance, defects in production lines may occur only after years of successful production~\cite{Wang_2022_BMVC}. Second, the available anomalies rarely represent all potential cases, as they are unexpected events. For instance, defects might be initially caused by the same event (i.e., they are similar to each other) and evolve over time because of changes in the production line.}

%First, collecting anomalies is often challenging because anomalous events are rare and sparse. For example, in autonomous driving, abnormalities such as sensor malfunctions or unexpected pedestrian movements are infrequent but can have severe consequences if not addressed. This rarity makes detecting and addressing such issues critical, especially in safety-critical systems. Second, the anomalies that are available rarely represent all potential cases because they arise from unforeseen events. For instance: in financial fraud detection, new techniques and schemes are constantly developed, meaning the anomalies previously identified do not encompass future fraudulent methods. These examples underscore the difficulty in obtaining comprehensive anomaly datasets, as new and unpredictable anomaly types are inherent to the very nature of these events.

Unfortunately, anomalies are inherently rare and sparse, which makes collecting them hard. 
As a result, the data used to train data-driven methods for anomaly detection only contains a limited number of anomalies.  
In autonomous driving, for instance, sensor malfunctions or unexpected pedestrian movements are infrequent but critical to address. As an additional challenge, available anomalies rarely represent all potential cases due to the unpredictable nature of these events. In financial fraud detection, new techniques and schemes are constantly emerging, meaning previously identified anomalies do not cover future fraudulent methods. These factors highlight the difficulty of obtaining comprehensive anomaly datasets, as new and unpredictable anomaly types are inherent to the very nature of these events.

%Because anomalies are rare, sparse, and unexpected, collecting anomalous examples is usually challenging. Moreover, the collected anomalies
%Moreover, the limited anomalies observed may be biased examples, i.e. they do not comprehensively represent all potential anomalous cases. For instance, defects might be initially similar to each other (e.g., they are caused by the same event) and evolve over time because of changes in the production line.

With recent improvements in generative modeling (e.g. ~\cite{ho2020denoising,dhariwal2021diffusion}) it seems natural to introduce auxiliary anomalies, e.g. for training an anomaly detector \citep{murase2022algan}, or for model selection ~\citep{fung2023model}.  However, there are several failure cases for generated anomalies that should not be neglected. For one, auxiliary anomalies might be too similar to normal examples. For instance, the defects introduced into images of products might be imperceptible, making the image indistinguishable from a normal counterpart. On the other hand, the quality of a generated anomaly also deteriorates as it becomes too unrealistic, e.g. when the generated defect of a product is too severe. Including poor-quality anomalies for training a model is likely to harm its performance~\cite{hendrycks2019oe,qiu2022latent,li2023deep,li2023zero}. Although \citet{chen2021atom,ming2022poem} proposed sampling methods for selecting informative anomalies during training, there is no approach for quantifying the quality of auxiliary anomalies.%, such that only high-quality examples would enrich the training set. \lorenzo{Definitely need more references...}



In this paper, we close this critical gap by introducing the \textbf{Expected Anomaly Posterior (\ourmethod{})}, the first example-wise score function that measures the quality of auxiliary anomalies. Our approach relies on a fundamental insight: high-quality auxiliary anomalies must fulfill two criteria — they must be (1) distinguishable from normal examples in the training data and (2) realistic, i.e. similar to the training examples (e.g., scratches only affect few pixels, leaving an anomalous image relatively similar to a normal one). Finding a balance between these two characteristics poses an inherent challenge. On one hand, auxiliary anomalies risk deteriorating an anomaly detector's performance if they closely resemble normal examples. On the other hand, they become less useful the more dissimilar from the training data.

Building upon this insight, we adopt a Bayesian framework to model the uncertainty of a detector's prediction. This framework accounts for both an example's dissimilarity from the normal class (via class-conditional probability) and its realism (via example density). The expectation of the posterior probability that an example is anomalous reflects our concept of the quality of an auxiliary anomaly: the approximation we derive in \Cref{sec:method} to compute the \ourmethod{} will give lower scores to indistinguishable and unrealistic anomalies.

%In summary, we make \lorenzo{X} contributions. First, we introduce the problem of evaluating the quality of an auxiliary set of anomalous examples. Second, we design the first metric that can capture the quality of a synthetic anomaly, where the higher the quality the higher its impact on the model's test performance when included in the training set. Third, we empirically show that \ourmethod{} outperforms several adapted baselines at measuring the quality of the anomalies. Finally, we experimentally show that including the high-quality auxiliary anomalies into the training set according to \ourmethod{} enhances the model's performance at test time. \lorenzo{we may want to add the prompt tuning part, if we'll use it}

% In summary, we make four contributions. First, we introduce the problem of evaluating the quality of an auxiliary set of anomalous examples. Second, we design the first metric that can capture the quality of an auxiliary anomaly, where the higher the quality more valuable it is for learning an anomaly detector. Third, we provide a theoretical analysis of \ourmethod{}'s convergence properties and its ranking guarantee. Fourth, we compare \ourmethod{} with nine baselines extensively on $40$ image and tabular datasets and demonstrate that \ourmethod{} enhances the model's performance by using high-quality auxiliary anomalies for training or model selection.

In summary, we make three following contributions. 
\begin{itemize}[nolistsep,leftmargin=*]
\item In \Cref{sec:method}, we compute the expected anomaly posterior (\ourmethod{}), which measures the quality of an anomaly by accounting both for aleatoric and epistemic uncertainty.
\item In \Cref{sec:theory}, we provide a theoretical analysis of \ourmethod{}, including its properties and guarantees. 
\item In \Cref{sec:exp}, we run an extensive experimental analysis and show that \ourmethod{} enhances a detector's performance when using high-quality anomalies to enrich training or perform model selection.
\end{itemize}

% First, we introduce the problem of evaluating the quality of an auxiliary set of anomalous examples. Second, we design the first metric that can capture the quality of an auxiliary anomaly, where the higher the quality more valuable it is for learning an anomaly detector. Third, we provide a theoretical analysis of \ourmethod{}'s convergence properties and its ranking guarantee. Fourth, we compare \ourmethod{} with nine baselines extensively on $40$ image and tabular datasets and demonstrate that \ourmethod{} enhances the model's performance by using high-quality auxiliary anomalies for training or model selection.



==> neurips2024/texfiles/methodology.tex <==
\section{Methodology}\label{sec:method}
In this Section, we introduce the problem setup and notations (\Cref{subsec:setup_and_notation}), and describe our proposed approach for quantifying the quality of auxiliary anomalies (\Cref{subsec:defake}).

\subsection{Problem setup}\label{subsec:setup_and_notation}
Let $(\Omega, \mathcal{F}, \Pp)$ be a probability space, and $X \colon \Omega \to \R^d$, $Y \colon \Omega \to \{0,1\}$ two random variables representing, respectively, feature vectors and class labels ($0$ for normals, $1$ for anomalies). A training dataset is an i.i.d. sample of pairs $D = \{(x_1,y_1), \dots, (x_n,y_n)\} \sim \Pp(X,Y)$ drawn from the joint distribution. Because of the rarity of anomalies, we assume to have only $m << n$ (labeled) examples from the anomaly class, in addition to $n-m$ (labeled) normal examples.
%In the semi-supervised setting, only few labels are given, and in the unsupervised setting, all labels are missing. 

Since anomalies provide valuable training signals, but are so rare to acquire, \citet{hendrycks2019oe,murase2022algan} propose using auxiliary anomalies during training. With significant improvements in generative modeling, there are many candidate methods for generating synthetic anomalies to complement the training data. Our goal is to evaluate candidate synthetic anomalies with a quality score function $\phi$ such that higher scores indicate that the synthetic anomaly is useful for training a detector. Before formalizing our research task, we introduce the following definition.
\begin{definition}[Categorization of Anomalies]\label{def:categorizationanomalies}
Given the examples $\xreal{}, \xunr{}, \xind{} \in \R^d$, we define that 
\begin{itemize}[nolistsep,noitemsep,leftmargin=*]
\item $\xreal{}$ is a \emph{realistic anomaly} if it has high conditional probability and non-zero density
\begin{equation*}
    \Pp(Y=1|X=\xreal{}) \in [0.5, 1] \ \text{ and } \ \Pp(X=\xreal{}) > 0;
\end{equation*}
\item $\xunr{}$ is an \emph{unrealistic anomaly} if it has high conditional probability and null density 
\begin{equation*}
    \Pp(Y=1|X=\xunr{}) \in [0.5, 1] \ \text{ and } \ \Pp(X=\xunr{}) = 0 ;
\end{equation*}
\item $\xind{}$ is an \emph{indistinguishable anomaly} if it has null conditional probability and non-zero density
\begin{equation*}
    \Pp(Y=1|X=\xind{}) = 0 \ \text{ and } \ \Pp(X=\xind{}) > 0.
\end{equation*}
\end{itemize}
\end{definition}


An anomaly detector is a function $f \colon \R^d \times \{0,1\} \to \R$ that assigns a real-valued anomaly score $f(x)$ to any $x \in \R^d$. The detector $f$ is learned using the training set $D$, and can be used for estimating the conditional probability $\Pp(Y|X)$ by mapping the scores to $[0,1]$~\cite{kriegel2011interpreting}.





%A quality metric is a function $\phi \colon \R^d \to \R$ such that, if $\phi(x,\Tilde{y})> \phi(\bar{x},\bar{y})$, then $f$ trained on $D\cup \{(x,\Tilde{y})\})$ is higher than trained on $D\cup\{(\bar{x},\bar{y})\})$.

\begin{description}
    \item[Given:] $D$ with $m \ll n$ anomalies, a set of $l$ auxiliary anomalies $\{x \in \R^d \}$ , and a detector $f$;
    \item[Challenge:] Design a quality score function $\phi : \R^d \to \R$ for the auxiliary anomalies, such that for any realistic anomaly $\xreal \in l$ and any unrealistic or indistinguishable anomaly $\xunr{},\xind{} \in l$, the realistic anomaly has a higher quality score $\phi(\xreal)> \phi(\xunr{}), \phi(\xind{})$.
\end{description}

With this categorization, estimators for $\Pp(Y|X)$ alone cannot differentiate between $\xreal{}$ and $\xunr{}$, while estimators for $\Pp(X)$ alone cannot differentiate between $\xreal{}$ and $\xind{}$, thus not qualifying as good quality estimators.
Intuitively, a score must quantify the conditional probability to distinguish between $\xreal{}$ and $\xind{}$ but the estimate needs to account for an example's density. Roughly speaking, the lower an example's density the more uncertain the estimate, because the lack of similar training data prevents a model from learning the correct probability. This introduces an additional level of uncertainty (namely, epistemic), which requires a Bayesian perspective to be properly measured~\cite{hullermeier2021aleatoric,bengs2022pitfalls}. 


%Designing a quality metric for synthetic auxiliary anomalies has two key challenges. 
%First, having access to a small and potentially biased set of $m$ anomalies makes the performance of a detector $f$ unreliable for distinguishing between realistic and unrealistic anomalies. 
%That is, the variation of utility for an example may not be indicative of its contribution to the test performance.
%Second, while existing data quality metrics retrain a model for each training example, doing so for an external set of anomalies might be prohibitively expensive, as one may want to evaluate a large set of auxiliary anomalies. Thus, the number of model trainings cannot scale with the size of the external set.
\subsection{The Expected Anomaly Posterior}\label{subsec:defake}




%if an anomaly detector has high uncertainty in predictions, the example is likely to be either too close (e.g., overlapping) to the normal training examples, or in an unexplored region (e.g., an out-of-distribution) of the example space. Specifically, an auxiliary anomaly falling into the normal region may indicate that it is indistinguishable from a normal counterpart, while a synthetic anomaly falling in an unexplored region is likely to be unrealistic to occur in practice.




%On the contrary, a quality metric that assigns high scores to real anomalies and low scores to unrealistic and indistinguishable anomalies needs to account for both. Intuitively, 

%(i) an example $x$'s conditional probability $\Pp(Y=1|X=x)$, which commonly reflects the underlying aleatoric uncertainty of the data, and (ii) an example $x$'s density $\Pp(X=x)$, which reflects the epistemic uncertainty~\cite{hullermeier2021aleatoric,bengs2022pitfalls}. Thus, \ourmethod{} focuses on quantifying a detector's total uncertainty.

%\paragraph{A Bayesian framework for uncertainty quantification.} C
Capturing a detector's uncertainty is challenging because one needs to account for (1) the example's proximity to the normal class (i.e., the aleatoric uncertainty) and (2) the lack of training data in the region where the example falls (i.e., the epistemic uncertainty). This is particularly complicated in anomaly detection because the epistemic uncertainty tends to be high for most anomalies, as they often fall in low-density regions~\cite{bengs2023second}.

We propose \ourmethod{}, a novel approach that estimates the quality of auxiliary anomalies by capturing an anomaly detector's uncertainty. The key idea is to model each example's probability of being an anomaly $p_x$. The quality score we propose is the expected posterior of this parameter.

\paragraph{Assumption.} For any $x$ the class conditional distribution $Y=1|X=x$ is a Bernoulli
\begin{equation*}
\Pp(Y|X=x) = \textsc{Bernoulli}(p_{x}), \quad p_{x} \sim \textsc{Beta}(\alpha_0,\beta_0).
\end{equation*}
The parameter $p_{x}$ can be interpreted as the probability of the example $x$ being an anomaly. With the Beta prior we can incorporate prior knowledge such as the expected ratio of anomalies in the data~\cite{perini2023estimating}.
Since we have at most one observation of $Y$ for each $x$, we follow \citet{charpentier2020posterior} and model the posterior over $p_x$ by conditioning on pseudo observations. 
Given $N$ pseudo observations $\bar{y}_1, \dots, \bar{y}_N$ hypothetically drawn from $\Pp(Y|X=x)$, the posterior,
\begin{equation}\label{eq:posterior_uncertainty}
    p_{x}| \bar{y}_1, \dots, \bar{y}_N \sim \textsc{Beta}(\alpha_0 + \alpha_1, \beta_0 + N - \alpha_1),
\end{equation}
is conjugate to the Beta prior, where $\alpha_1 = \sum_{i=1}^N \1 (\bar{y}_i=1)$ is the number of anomalies in the pseudo observations. That is, if we could sample $N$ labels for the same example $x$, i.e. $(x, y_1),\dots, (x, y_N)$, we would derive the posterior distribution of $Y|X=x$ by using a simple Bayes update (Eq.~\ref{eq:posterior_uncertainty}). However, sampling $N$ labels for the same example $x$ is practically impossible. Thus, we need to parametrize $\alpha_1$. Roughly speaking, if we drew $n$ training examples from $\Pp(X,Y)$ we would expect to draw $N = n \cdot \Pp(X=x)$ examples with features $x$, among which $\Pp(Y=1|X=x)$ are anomalies:
%which represents \emph{the expected number of labels drawn from $Y|X=x$ and belonging to the positive class, if we spread a budget of $N$ labels over the example space. Roughly speaking, if we drew $N$}:}
\begin{equation}
    \alpha_1 \approx n \times \reallywidehat{\Pp(Y\!=\!1,X\!=\!x)} \approx n \times \underbrace{\reallywidehat{\Pp(Y\!=\!1|X\!=\!x)}}_{\text{conditional probability}} \times \underbrace{\reallywidehat{\Pp(X\!=\!x)}}_{\text{data density}} 
\end{equation}
where $\hat{\cdot}$ indicates that the quantity is estimated. We describe how we compute both terms below. 
The expectation of the posterior in \Cref{eq:posterior_uncertainty} reflects the quality of an auxiliary anomaly $x$: if the expected posterior is high, the evidence is enough to rely on the expected conditional probability for evaluating the auxiliary anomaly, while if it is low, the quality reflects our prior belief.

\paragraph{Estimating the data density.}
Computing $\reallywidehat{\Pp(X\!=\!x)}$ has two main challenges. First, most traditional density estimators suffer the well-known curse of dimensionality~\cite{verleysen2005curse,bengio2005curse}. Second, deep estimators (e.g., Normalizing Flows~\cite{kobyzev2020normalizing}) are prohibitively time-consuming to be employed for data quality scores. Thus, \ourmethod{} relies on the rarity score~\cite{han2022rarity}, which is fast to compute and weakly affected by the curse of dimensionality. 
The rarity score (1) creates k-NN spheres centered on each training example, and (2) assigns the smallest radius of the sphere that contains the given synthetic example. If the synthetic example falls outside of all spheres, it is considered too uncommon and gets null rarity. 
% We use the rarity score $r_{\hat{k}}$ with an estimated $k$ to estimate the data density as 

% Formally, given a synthetic image with extracted feature $x$, the rarity score is a function $r_k \colon \R^d \to \R$ such that 
% \begin{equation}
% r_k(x) = 
% \begin{cases}
%     0  &\text{if } x \notin \!\!\bigcup\limits_{x_i \in D} \!\! B_k(x_i)\\
%     \min\limits_{x_i \in D \colon x \in B_k(x_i)} \!\! NN_k(x_i) &\text{otherwise}
% \end{cases}
% \end{equation}
% where $NN_k(x_i)$ is the distance between $x_i$ and its k-th nearest neighbor in $D$, and $B_k(x_i) = \{x|d(x_i,x) \le NN_k(x_i)\}$ is the k-NN sphere with $x_i$ as center and $NN_k(x_i)$ as radius. The rarity score strongly depends on the choice of the hyperparameter $k$: high values of $k$ could map far unrealistic examples to a positive high score, namely they would be considered authentic, while low values of $k$ could map real examples slightly different than the training data to a null score, namely they would be considered artifacts.


% Because the rarity score strictly depends on the hyperparameter $k \in \{1,\dots, n-1\}$, we need to estimate a proper value $\hat{k}$. Let's assume the existence of an optimal $k$, and use the small set of $m$ anomalies to estimate it.
% Ideally, $k$ should be: (1) as low as possible to assign null scores to unrealistic anomalies, and (2) high enough to assign positive scores to the real training anomalies. 

% Following this insight, we assume a Bayesian perspective and set a normalized variable's $K$ prior to be uniform
% \begin{equation*}
%     K \coloneqq \frac{k-1}{n-1} \sim \textsc{Beta}(1,1) = \textsc{Unif}(0,1).
% \end{equation*}
% Roughly speaking, we min-max normalize $K$ to $[0,1]$ to exploit that a Beta prior with a Bernoulli likelihood results in a Beta posterior distribution. Because we want the minimum $k$ that assigns positive scores to the training anomalies $\{x_{\bar{m}}\}_{\bar{m}\le m}$, we compute for each $x_{\bar{m}}$ the minimum $k_{\bar{m}}$ such that $r_{k_{\bar{m}}}(x_{\bar{m}})>0$. The set of normalized $\{\frac{k_{\bar{m}}-1}{n-1}\}_{\bar{m}\le m}$ is the empirical evidence for the Bayesian update, which is
% \begin{equation*}
%     K\Big|\!\left\{\!\frac{k_{\bar{m}}\!-\!1}{n\!-\!1}\!\right\}\! \sim \!\textsc{Beta}\!\!\left(\!\!1\!+\!\!\!\sum_{\bar{m}\le m}\!\! \frac{k_{\bar{m}}\!-\!1}{n\!-\!1}, 1\! +\! m\! -\!\!\! \sum_{\bar{m}\le m} \!\!\frac{k_{\bar{m}}\!-\!1}{n\!-\!1}\!\right)\!.
% \end{equation*}
% Finally, we estimate $\hat{k}$ as the $95$th percentile of the posterior distribution of $K$
% \begin{equation}
%     \hat{k} = \argmin_{t\in[0,1]} \Pp\left(K\Big|\left\{\frac{k_{\bar{m}}-1}{n-1}\right\} \le t\right) \ge 0.95
% \end{equation}
% which guarantees that at least $95\%$ of real anomalies get a positive rarity score.
We use the rarity score $r_{\hat{k}}$ with an estimated $\hat{k}$ to estimate the data density.\footnote{We explain how we compute $\hat{k}$ in \Cref{sec:rarity_score} in the Supplement.}
Intuitively, the density behaves as the inverse of the rarity score: highly uncommon examples should have low density. Thus, we take the reciprocal value of the rarity score and normalize it using the training rarity scores:
\begin{equation}\label{eq:density}
    \reallywidehat{\Pp(\!X\!=\!x\!)} = \frac{1 \slash r_{\hat{k}}(x)}{1 \slash r_{\hat{k}}(x)+\sum_{i=1}^n 1 \slash r_{\hat{k}}(x_i)}.
\end{equation}

\paragraph{Estimating the conditional probability.}
Computing $\reallywidehat{\Pp(Y\!=\!1|X\!=\!x)}$ in anomaly detection is a hard task because (1) class probabilities are generally unreliable for imbalanced classification tasks~\cite{wallace2012class,tian2020posterior}, and (2) the available anomalies might be non-representative of the whole anomaly class (i.e., we have access to a biased set). This makes traditional calibration techniques often impractical~\cite{silva2023classifier,deng2022cadet}. However, we mainly care about having probabilities that satisfy two properties. First, they must be coherent with the detector's prediction, namely a predicted anomaly (normal) needs a probability greater (lower) than $0.5$. Second, we want the proportion of predicted anomalies to match the expected proportion of true anomalies. This guarantees that, if the detector's ranking is accurate, the class predictions are optimally computed.

For this task, we employ a squashing scaler~\cite{vercruyssen2018semi} to map the anomaly scores to $[0,1]$ probability values
\begin{equation}\label{eq:classconditionaprob}
\reallywidehat{\Pp(\!Y\!=\!1|X\!=\!x\!)} = 1-2^{-\left(\frac{f(x)}{\lambda}\right)^2}
\end{equation}
where $\lambda$ is the detector's decision threshold which we set such that the number of training examples with probability $> 0.5$ (after mapping) is equal to the number of training anomalies $m$~\cite{perini2023estimating}.

\paragraph{Computing the quality scores.} Using our point estimates for the data density and the conditional probability, the parametrized posterior distribution $p_{x}| \bar{y}_1, \dots, \bar{y}_N$ can be computed by substituting $\alpha_1 = n \reallywidehat{\Pp(Y\!=\!1|X\!=\!x)} \reallywidehat{\Pp(X\!=\!x)}$ and $N = n \reallywidehat{\Pp(X\!=\!x)}$ to Eq.~\ref{eq:posterior_uncertainty}. Finally, we compute the quality of an auxiliary anomaly $x$ by taking its expectation
\begin{align*}
\phi(x) = \E[p_{x}| \bar{y}_1, \dots, \bar{y}_N] = \frac{\alpha_0 + n \reallywidehat{\Pp(X=x)} \reallywidehat{\Pp(Y=1|X=x)}}{\alpha_0 + \beta_0 + n \reallywidehat{\Pp(X=x)}}.
\end{align*}



==> neurips2024/texfiles/preliminaries.tex <==
\section{Related Work}
\paragraph{Anomaly detection.} Designing an anomaly detector requires developing a way to assign real-valued anomaly scores to the examples~\cite{chandola2009anomaly,han2022adbench}, where the higher the score, the more anomalous the example. Existing approaches often rely on heuristic intuitions about expected anomalous behavior~\cite{pang2021deep,qiu2023self}. Propagation-based detectors, such as those using proximity to training examples, assume similar instances share the same label (e.g., \textsc{SSDO})~\cite{vercruyssen2018semi}. Loss-based detectors, on the other hand, learn a decision boundary (e.g., a hypersphere over normals) and assign scores based on the distance to this boundary~\cite{ruff2019deep,zhou2021feature,gao2021connet,Qiu2022RaisingTB}. Self-supervised detectors learn models through solving auxiliary tasks and score anomalies according to model performance on self-supervised tasks~\cite{golan2018deep,bergman2020classification,qiu2021neural}. Recently, foundation models have enabled zero-shot anomaly detection~\cite{jeong2023winclip}, which overcomes the need to collect anomalies for training but still requires their use in model selection~\cite{fung2023model}.




%\paragraph{Deep anomaly detection.} Designing an anomaly detector requires developing a way to assign real-valued anomaly scores to the examples~\cite{chandola2009anomaly,han2022adbench}, where the higher the score, the more anomalous the example. Normally, detectors rely on heuristic intuitions on the expected anomalous behavior~\cite{pang2021deep,qiu2023self}. For instance, propagation-based detectors assume that similar instances share the same label and assign scores based on the proximity to training examples~\cite{vercruyssen2018semi,deng2022ssdbcodi}. Loss-based detectors separate normals and anomalies by learning a decision boundary (e.g., a hypersphere over the normals) and assign scores according to the distance to such a boundary~\cite{ruff2019deep,zhou2021feature,gao2021connet,Qiu2022RaisingTB}. Alternatively, self-supervised anomaly detection methods learn the model by solving auxiliary learning problems and assign scores according to the model performance on the self-supervised task~\cite{golan2018deep,bergman2020classification,qiu2021neural}. Recently, the success of foundation models has enabled zero-shot anomaly detection~\cite{jeong2023winclip}. While this no longer requires collecting anomalies for model training, one still needs to leverage them for model selection~\cite{fung2023model}. 

%Another pioneering stream of research has shown that anomaly detectors' performance improves when exposed to more high-quality anomalies~\cite{hendrycks2019oe,qiu2022latent,li2023deep,li2023zero}. Although \citet{chen2021atom} and \citet{ming2022poem} proposed greedy-based sampling methods for selecting informative anomalies in training, no approach can quantify the quality of auxiliary anomalies.


\paragraph{Data quality.} Traditional quality score functions evaluate training examples by (1) defining a utility function that takes as input a subset of the training set and measures the performance of the model, and (2) finding a function that assigns a score to an example by quantifying its impact on the model's performance when included/excluded for training~\cite{yoon2020data,jiang2023opendataval}. Methods like leave-one-out (\textsc{Loo}) iteratively remove one example at a time to observe how test performance varies. Various techniques, such as \textsc{DataShap}~\cite{ghorbani2019data}, \textsc{BetaShap}~\cite{kwon2021beta}, \textsc{KNNShap}~\cite{jia2019efficient}, \textsc{DataBanzhaf}~\cite{wang2023data}, and \textsc{AME}~\cite{lin2022measuring}, compute the marginal contribution of an example by bootstrapping the training set and assessing its impact on model training. \textsc{DataOob} is an out-of-bag (OOB) evaluator that measures out-of-bag accuracy variation. Other methods like \textsc{Lava} and influence functions (\textsc{Inf}) quantify how the utility changes when a specific example is more weighted. The Supplement~\ref{sec:data_quality_estimators} provides a detailed overview. Unfortunately, all existing data quality estimators focus on evaluating the impact of training examples and are not tailored to estimate the quality of an external anomaly.


%\paragraph{Data valuation.} Traditional data quality metrics evaluate training examples by (1) defining a utility function that takes as input a subset of the training set and measures the performance of the model, and (2) finding a function that assigns a score to an example by quantifying its impact on the model's performance when included/excluded for training~\cite{yoon2020data,jiang2023opendataval}. For instance, leave-one-out (\textsc{Loo}) removes one example at a time from the training set to measure how the test performance varies. Several methods such as \textsc{DataShap}~\cite{ghorbani2019data}, \textsc{BetaShap}~\cite{kwon2021beta}, \textsc{KNNShap}~\cite{jia2019efficient}, \textsc{DataBanzhaf}~\cite{wang2023data}, and \textsc{AME}~\cite{lin2022measuring} compute the marginal contribution of an example by bootstrapping the training set and measuring the impact of an example when included/excluded in the bootstraps used for training the model. Alternatively, \textsc{DataOob}~\cite{kwon2023data} is an out-of-bag (OOB) evaluator that measures the variation of the out-of-bag accuracy, namely the accuracy of the prediction on the non-selected examples in the bootstrap. Finally, methods like \textsc{LavaEvaluator}~\cite{just2023lava} and influence functions (\textsc{Inf})~\cite{feldman2020neural} quantify the rate at which a utility value changes when a particular example is more weighted. Unfortunately, all existing data quality metrics target evaluating the impact of training examples, and none of them are tailored to estimating the quality of an external anomaly.

% Recently, \citet{han2022rarity} proposed to measure the rarity (i.e., the uncommonness) of synthetic images to evaluate the ability of a generative model to create authentic images. Roughly speaking, the rarity score (1) creates k-NN spheres centered on each training example, and (2) assigns the smallest radius of the sphere that contains the given synthetic example. If the synthetic example falls outside of all spheres, it is considered too uncommon and gets a rarity equal to $0$. Formally, given a synthetic image with extracted feature $\Tilde{x}$, the rarity score is a function $r_k \colon \R^d \to \R$ such that 
% \begin{equation}
% r_k(\Tilde{x}) = 
% \begin{cases}
%     0  &\text{if } \Tilde{x} \notin \!\!\bigcup\limits_{x_i \in D} \!\! B_k(x_i)\\
%     \min\limits_{x_i \in D \colon \Tilde{x} \in B_k(x_i)} \!\! NN_k(x_i) &\text{otherwise}
% \end{cases}
% \end{equation}
% where $NN_k(x_i)$ is the distance between $x_i$ and its k-th nearest neighbor in $D$, and $B_k(x_i) = \{x|d(x_i,x) \le NN_k(x_i)\}$ is the k-NN sphere with $x_i$ as center and $NN_k(x_i)$ as radius. The rarity score strongly depends on the choice of the hyperparameter $k$: high values of $k$ could map far unrealistic examples to a positive high score, namely they would be considered authentic, while low values of $k$ could map real examples slightly different than the training data to a null score, namely they would be considered artifacts.



==> neurips2024/texfiles/theory.tex <==
\section{Theoretical Analysis of \ourmethod{}}
\label{sec:theory}
We theoretically investigate two tasks. First, we illustrate the main properties of \ourmethod{}, namely how it behaves when subject to (1) large training sets ($n \to +\infty)$, (2) small training sets or zero-density examples, (3) high-class conditional probabilities.
Second, we answer the following question: \emph{Given a realistic anomaly $\xreal{}$, an indistinguishable anomaly $\xind{}$ and an unrealistic anomaly $\xunr{}$ as in \Cref{def:categorizationanomalies}, does \ourmethod{} rank $\phi(\xreal{})>\phi(\xind{}),\phi(\xunr{})$?
}

\subsubsection*{i) \bf{\ourmethod{} has three relevant properties:}}

\emph{P1) Convergence to class conditional probabilities.} The number of training examples indicates how strong the empirical evidence is. That is, the detector $f$ has enough evidence to estimate properly the class conditional probability. Thus, for high $n$, \ourmethod{} converges to the class conditional probability
\begin{equation*}
    \phi(x) \to \reallywidehat{\Pp(Y\!=\!1|X\!=\!x)} \qquad \text{for } n \to +\infty;
\end{equation*}


\emph{P2) Convergence to the prior's mean.} No empirical evidence implies that the posterior remains equal to the prior. Thus, \ourmethod{} assigns the prior's mean for relatively small $n$ or a null-density region, 
\begin{equation*}
    \phi(x) \to \frac{\alpha_0}{\alpha_0+\beta_0} \qquad \text{for } n \to 0 \ \text{ or } \ \reallywidehat{\Pp(X=x)} \to 0.
\end{equation*}


\emph{P3) The quality of distinguishable anomalies increases with their density.} Given $\reallywidehat{\Pp(Y=1|X=x)} \approx 1$ for an example $x$, its quality depends only on its density: the closer/more similar to the training examples, the higher the density, the higher its quality:
\begin{equation*}
    \phi(x) \approx 1 - \frac{\beta_0}{\alpha_0+\beta_0 + n\Pp(X=x)}.
\end{equation*}


\subsubsection*{ii) \bf{\ourmethod{}' ranking guarantee.}}
We show that \ourmethod{} ranks the anomalies as (1st) realistic, (2nd) unrealistic, and (3rd) indistinguishable.

\begin{theorem}
Let $\xreal{}, \xunr{}, \xind{} \in \R^d$ be, respectively, a realistic, unrealistic, and indistinguishable anomaly. If the estimators in Eq.~\ref{eq:density} and Eq.~\ref{eq:classconditionaprob} satisfy the properties of \Cref{def:categorizationanomalies}, then
\begin{equation}
\frac{\alpha_0}{\alpha_0+\beta_0}<0.5 \implies \phi(\xreal{})>\phi(\xunr{}) > \phi(\xind{}).
\end{equation}
\end{theorem}
\begin{proof}
Using the definition of indistinguishable and unrealistic anomaly, we immediately conclude
\begin{equation*}
    \phi(\xunr{}) = \frac{\alpha_0}{\alpha_0+\beta_0} >  \frac{\alpha_0}{\alpha_0+\beta_0 + n\Pp(X=\xind{})} = \phi(\xind{})
\end{equation*}
because $\Pp(X=\xind{})>0$. As a second step, we assume that $\frac{\alpha_0}{\alpha_0+\beta_0}<0.5$ and show algebraically that
\begin{equation*}
\begin{split}
&\phi(\xreal{})>\phi(\xunr{}) \!\iff \!\phi(\xreal{})-\phi(\xunr{})>0  \!\iff \!\frac{\alpha_0 + n \Pp(X\!=\!\xreal{}) \Pp(Y\!=\!1|X\!=\!\xreal{})}{\alpha_0 + \beta_0 + n \Pp(X\!=\!\xreal{})}\!-\!\frac{\alpha_0}{\alpha_0+\beta_0}\!>\!0  \\
&\iff n\Pp(X\!=\!\xreal{})\left[(\alpha_0+\beta_0)\Pp(Y\!=\!1|X\!=\!\xreal{}) \!-\! \alpha_0\right]\!>0 \iff \Pp(Y\!=\!1|X\!=\!\xreal{}) > \frac{\alpha_0}{\alpha_0+\beta_0},
\end{split}
\end{equation*}
which holds as $\Pp(Y\!=\!1|X\!=\!\xreal{})>0.5> \frac{\alpha_0}{\alpha_0+\beta_0}$.
\end{proof}






==> texfiles/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
%The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page limit. 

%Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
%\begin{itemize}
%    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
%\end{itemize}

%{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

%The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

%IMPORTANT, please:
%\begin{itemize}
%    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
%\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We make two claims. First, we claim that our approach outperforms 12 baselines in the majority of cases, which we show in \Cref{sec:exp}. Second, we claim that our method ranks the anomalies as (1st) realistic, (2nd) unrealistic, and (3rd) indistinguishable, which we show in \Cref{sec:theory}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We detailed the key assumptions of the methodology in \Cref{sec:method} and \Cref{sec:theory}, as well as the general limitations in \Cref{sec:conclusion_and_limitations}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by , \answerNo{}, or \answerNA{}.
    \item[] Justification: \Cref{sec:theory} illustrates our main result and provides a complete proof. The properties can be quickly derived from basic calculus and limits.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \Cref{sec:exp} gives all details on our experimental setup, including the preprocessing of the data, the model's hyperparameters, and the procedure to correctly set the experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We will release the code upon acceptance. The data is publicly available. The experimental section provides all the details to reproduce the results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \Cref{sec:exp} provides all details.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \Cref{tab:mean_pm_std} in the Supplement shows the aggregated results in terms of mean $\pm$ standard deviation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \Cref{sec:exp} (setup) gives all details.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We are aware of the code of ethics and do not violate any clause.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \Cref{sec:conclusion_and_limitations} provides our statement on the societal impact.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not have risks for misuse to the best of our knowledge.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Only the authors contributed to this paper. The license has been selected for submission in OpenReview.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Code will be released upon acceptance, along with the framework to use it.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


==> texfiles/packages.tex <==
\usepackage{mathrsfs}
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{booktabs} % for professional tables
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{enumitem}
\usepackage[capitalize,noabbrev]{cleveref}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\usepackage[textsize=tiny]{todonotes}

\newcommand{\ourmethod}[0]{\textsc{EAP}}
\usepackage{dsfont}

\newcommand{\numberset}{\mathbb} %
\newcommand{\N}{\numberset{N}}
\newcommand{\Z}{\numberset{Z}}
\newcommand{\R}{\numberset{R}}
\newcommand{\C}{\numberset{C}}
\newcommand{\E}{\numberset{E}}
\newcommand{\1}{\mathds{1}}
\newcommand{\Pp}{\mathbb{P}}
\newcommand{\Ss}{\mathcal{S}}
\newcommand{\Yy}{\mathcal{Y}}
\newcommand{\Chi}{\mathcal{X}}
\newcommand{\Qq}{\mathcal{Q}}
\newcommand{\xreal}{x_{\textsc{r}}}
\newcommand{\xind}{x_{\textsc{i}}}
\newcommand{\xunr}{x_{\textsc{u}}}
\newcommand{\xui}{x}


\newcommand{\lorenzo}[1]{\textcolor{violet}{[LP: #1]}}
\newcommand{\chen}[1]{\textcolor{green}{[CQ: #1]}}
\newcommand{\maja}[1]{\textcolor{blue}{[MR: #1]}}

\newcommand{\changed}[1]{\textcolor{orange}{#1}}

\usepackage{scalerel,stackengine} %for the hat above math 
\stackMath
\newcommand\reallywidehat[1]{%
\savestack{\tmpbox}{\stretchto{%
  \scaleto{%
    \scalerel*[\widthof{\ensuremath{#1}}]{\kern-.6pt\bigwedge\kern-.6pt}%
    {\rule[-\textheight/2]{1ex}{\textheight}}%WIDTH-LIMITED BIG WEDGE
  }{\textheight}% 
}{0.5ex}}%
\stackon[1pt]{#1}{\tmpbox}%
}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\usepackage{tcolorbox}
